Direct observation of topological charge impacting skyrmion bubble stability in Pt/Ni/Co asymmetric superlattices

We characterize the magnetic properties and domain structure of Pt/Ni/Co asymmetric superlattices in comparison to the more established Pt/Co/Ni structure. This reversal in stacking sequence leads to a marked drop in interfacial magnetic anisotropy and the magnitude of the interfacial Dzyaloshinskii-Moriya interaction (DMI) as inferred from the DW structure, which we speculate could be related to a degradation of the Pt/Co interface when Pt is deposited on top of the Co layer. Lorentz transmission electron microscopy reveals exclusively N\'eel type domain walls and, with a perpendicular field, N\'eel skyrmions in the Pt/Co/Ni films. Conversely, the Pt/Ni/Co samples show only achiral Bloch domain walls, which leads to the formation of achiral Bloch ($Q=1$) and type II bubbles ($Q=0$) at increased perpendicular field. Combined with the reduced anisotropy leading to greater bubble densities, the latter case makes for an excellent test bed to examine the benefits of topological charge on stability. Simultaneous observation of Bloch and type II bubbles shows a roughly 50 mT larger annihilation field for the former. An in-plane component to the magnetic field is shown to both impact the structure of the formed bubbles and separately suppress the topological benefit.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
